A Geometric Approach to Constrained Online Learning

We study constrained online convex optimization with adversarial time-varying constraints. At each round the learner acts before observing the loss and constraint, and is compared with the best fixed action satisfying all constraints in hindsight. The goal is to obtain minimax-optimal regret while controlling cumulative constraint violation (CCV). Prior algorithms achieved $O(\log T)$ regret with $O(\sqrt{T\log T})$ CCV for strongly convex losses, and $O(\sqrt{T})$ regret with $O(\sqrt{T}\log T)$ CCV for convex losses. We present NP-OGD, an iterated nested-projection algorithm. For strongly convex losses it achieves $O(\log T)$ regret and $O(\log T)$ CCV; for convex losses it achieves $O(\sqrt{T})$ regret and $O(\sqrt{T})$ CCV. The analysis relies on a geometric movement bound: after lifting the nested projected-gradient trajectory to one higher dimension, the lifted path is self-contracted under a nonstandard norm, so a finite-length theorem for self-contracted curves controls the total projection movement. We also prove complementary lower bounds using layered sphere packings. For strongly convex losses, any online algorithm with polynomially sublinear regret can incur CCV at least $\Omega((\log T)^{(d-1)/(d+1)}/\log\log T)$. For convex losses, we prove CCV lower bounds $\Omega(T^{(d-1)/(2(d+3))})$ for weakly adaptive algorithms and $\Omega(T^{(d-1)/(2d)})$ for NP-OGD. Finally, for the constrained experts special case over $N$ experts, an active Hedge algorithm attains $O(\sqrt{T\log N})$ regret and $O(N)$ CCV, with a matching minimax CCV lower bound for sufficiently large horizons.

==> str-cvx-lb.tex <==
%\subsection{A Cone-Cap Lower Bound}
%\label{sec:cone-cap-lower-bound}
%
%We give a high-dimensional lower-bound construction based on well-separated
%cones, or equivalently, small caps of the Euclidean ball.  The construction is
%geometrically simple: each phase makes one cap attractive through the loss, and
%then, once the learner enters that cap, the adversary cuts it off while
%preserving all other caps.  Thus the adversary can repeat the same operation
%for many almost-orthogonal directions.
\iffalse
Let \(X\subseteq\mathbb R^d\) be the decision set.  For a COCO instance, define
the static regret
\[
        \Reg_T
        :=
        \sum_{t=1}^T f_t(x_t)
        -
        \min_{x\in S_T}\sum_{t=1}^T f_t(x),
\]
where
\[
        S_T
        =
        X\cap\bigcap_{t=1}^T\{x:g_t(x)\le0\},
\]
and define the cumulative constraint violation
\[
        \CCV_T
        :=
        \sum_{t=1}^T (g_t(x_t))_+.
\]

For a problem class \(\mathcal P\), define the regret-budget
value
\[
        V_{\mathcal P}(\mathcal R,T)
        :=
        \inf_{\mathcal A:\ \sup_{I\in\mathcal P}\Reg_T(\mathcal A,I)\le
        \mathcal R(T)}
        \sup_{I\in\mathcal P}\CCV_T(\mathcal A,I),
\]
where the infimum is over all online algorithms.





\subsection{A Spherical Cap-Separation Lemma}
In this Section, we establish a lemma showing that there are many non-overlapping spherical caps in high-dimensions. We will restrict our attention to the following setup.
\paragraph{Setup:}
For some suitable parameters \(0 \leq \rho, \delta \leq 1\) to be fixed later, define $\beta:=\rho+\sqrt{2\delta},$ where we require 
        $1- \delta - \beta >0$.
        
Let \(u_1,\ldots,u_M\in\mathbb S^{d-1}\) be $M$ unit vectors satisfying the approximate orthogonality criterion: 
\[
        |\langle u_i,u_j\rangle|\le \rho,
        \qquad
        i\neq j.
\]
Choose the decision set $\mathcal{X}$ to be the standard $d$-dimensional Euclidean ball. 
%Let \(r>0\), and let
%\[
%        X:=B(0,r).
%\]
For each \(j\in[M]\), define the spherical cone 
\[
        C_j
        :=
        \{x\in \mathcal{X}:\langle u_j,x\rangle\ge 1-\delta\}.
\]
Finally, for each \(i\in[M]\), define the halfspace
\[
        H_i
        :=
        \{x \in \mathcal{X}:\langle u_i,x\rangle\le \beta\}.
\]
%\cmt{Draw a figure}. 


\begin{lemma}[Spherical Cap separation]
\label{lem:cone-cap-separation}
In the above setup, we have 
\[ C_j\subseteq H_i ~~\forall i\neq j, \quad \textrm{and} \quad 
        C_i\cap H_i=\emptyset, ~\forall i.
\]
Consequently, the halfspace \(H_i\) removes the cap \(C_i\) while preserving
every other cap \(C_j\), \(j\neq i\).
\end{lemma}

\begin{proof}
Fix \(i\neq j\), and choose any \(x\in C_j\).  Then, by definition
\[
        \lnorm x\rnorm \le1,
        \qquad
        \langle u_j,x\rangle\ge1-\delta.
\]
Therefore
\[
\begin{aligned}
        \|x-u_j\|^2
        =
        \|x\|^2+\|u_j\|^2-2\langle x,u_j\rangle
        \le
        1+1-2(1-\delta)
        =
        2\delta.
\end{aligned}
\]
Thus we have that
\[
        \|x-u_j\|\le\sqrt{2\delta}.
\]
Finally, using the approximate-orthogonality of the vectors $\{u_i\}_{i=1}^M$, we have
\[
\begin{aligned}
        \langle u_i,x\rangle
        =
        \langle u_i,u_j\rangle+\langle u_i,x-u_j\rangle
        \le
        |\langle u_i,u_j\rangle|+\|x-u_j\|
        \le
        \rho+\sqrt{2\delta}
        =
        \beta.
\end{aligned}
\]
%Multiplying by \(r\), we obtain
%\[
%        \langle u_i,x\rangle\le r\beta.
%\]
Thus \(x\in H_i\), and hence, \(C_j\subseteq H_i, \forall i \neq j\).

On the other hand, every \(x\in C_i\) satisfies
\[
        \langle u_i,x\rangle\ge 1-\delta > \beta.
\]
%Since
%\[
%        \beta<1-\delta,
%\]

Thus no point in \(C_i\) belongs to \(H_i\), \emph{i.e.},  $C_i\cap H_i=\emptyset$.

\end{proof}
\fi


Let \(\mathcal P_{\rm cap}(d)\) denote the class of $\COCO$instances on the standard $d$-dimensional Euclidean ball with $1$-Lipschitz and convex loss and constraint functions. 

\begin{theorem}[$\CCV$ lower bound]
\label{thm:cone-cap-lower-bound}
%Fix \(D,G_f,G_g>0\).  Let \(\rho,\delta>0\) satisfy
%\[
%        \rho+\sqrt{2\delta}<1-\delta,
%\]
%and define
%\[
%        \nu:=1-\delta-\rho-\sqrt{2\delta}>0.
%\]
%Suppose there exist unit vectors
%\[
%        u_1,\ldots,u_M\in\mathbb S^{d-1}
%\]
%such that
%\[
%        |\langle u_i,u_j\rangle|\le\rho,
%        \qquad
%        i\neq j.
%\]
Consider the above setup. Fix any online $\COCO$algorithm achieving a regret budget of \(R(T)\ge0\) for all instances. Then there exists a $\COCO$problem instance for which, the minimax $\CCV$, defined in \eqref{reg-bud-lb}, is lower bounded as
\[
        V(R(T),T)
        \ge
        \nu
        \min\left\{
            M,\,
            \left\lfloor
            \log_{B_\delta}
            \left(
                \frac{T}{R(T)+1}
            \right)
            \right\rfloor_+
        \right\},
\]
where
\[
        B_\delta:=2+\frac{4}{\delta},
        \qquad
        \lfloor a\rfloor_+:=\max\{0,\lfloor a\rfloor\}, \qquad~\textrm{and}~~~ \nu = 1-\delta -\beta.
\]
In particular, if
$
        T\ge
        B_\delta^M
        \left(
            R(T)+1
        \right),
$
then the $\CCV$ is lower bounded as
$
        V(R(T),T)
        \geq 
        \Omega(M_{\rho, \delta}).
$
\end{theorem}

\begin{proof}
Fix an online $\COCO$algorithm \(\mathcal A\) with the standard $d$-dimensional Euclidean ball being its decision set $\mathcal{X}.$ Assume that $\mathcal{A}$ satisfies the regret budget
\[
        \sup_{I\in\mathcal P_{\rm cap}(d)}\Reg_T(\mathcal A,I)
        \le
         R(T).
\]
%Let
%\[
%        r:=\frac D2,
%        \qquad
%        X:=B(0,r).
%\]
%Then \(X\) has diameter \(D\).
%
%Let
%\[
%        \beta:=\rho+\sqrt{2\delta}.
%\]
Recall the definition of the spherical caps and the half-spaces
\begin{eqnarray} \label{feas-set2}
        C_j
        :=
        \{x\in \mathcal{X}:\langle u_j,x\rangle\ge 1-\delta\}, \quad  H_j
        :=
        \{x \in \mathcal{X}:\langle u_j,x\rangle\le \beta\}, ~\forall j \in [M],
\end{eqnarray}
where  $\beta:=\rho+\sqrt{2\delta}.$
%For each \(j\in[M]\), define
%\[
%       
%\]
By Lemma~\ref{lem:cone-cap-separation}, the cut \(H_j\) removes \(C_j\) while
preserving every other cap \(C_i\), \(i\neq j\).

Let
\[
        m
        :=
        \min\left\{
            M,\,
            \left\lfloor
            \log_{B_\delta}
            \left(
                \frac{T}{\mathcal R(T)+1}
            \right)
            \right\rfloor_+
        \right\}.
\]
If \(m=0\), there is nothing to prove.  So we assume \(m\ge1\).

We recursively construct a hard problem instance with \(m\) phases.  At the beginning of phase \(j\),
the cap \(C_j\) is still feasible as only caps \(C_1,\ldots,C_{j-1}\) have been removed, and Lemma~\ref{lem:cone-cap-separation} says that all
previous cuts preserve \(C_j\).

Phase $j$ begins at round $P_j+1$ (we set  
        $P_1:=0$) and continues for $L_j$ rounds unless it ends prematurely due to the learner playing an action from the set $C_j.$
The nominal length $L_j$ of the $j$\textsuperscript{th} phase is given by 
\begin{eqnarray} \label{lj-def}
        L_j
        :=
        \left\lceil 
        \frac{ 4(R(T)+P_j+1) }
        {\delta}
        \right\rceil,
        \qquad
        P_{j+1}\leq P_j+L_j.
\end{eqnarray}
%Thus phase \(j\) consists of rounds
 %       $P_j+1,\ldots,P_{j+1}.$

During phase \(j\), as long as the learner has not yet played an action from the cap \(C_j\), the
adversary reveals the linear loss function
\begin{eqnarray} \label{loss-fun-phasej}
        f_t(x):=-\langle u_j,x\rangle	
\end{eqnarray}

and the trivial constraint
\[
        g_t(x)\equiv0
\]
at each round during phase $j$. We now make the following claim. 
%The loss is convex and \(G_f\)-Lipschitz.
\begin{claim} \label{claim}
A no-regret learner must play an action from the spherical cap $C_j,$ defined in Eqn.\ \eqref{feas-set}, during phase $j.$
\end{claim}
\begin{proof}
Suppose, for the sake of contradiction, that the learner does not play any action from the spherical cap \(C_j\) during phase \(j\). Then for each round \(t\) in phase \(j\), we have 
\[
        \langle u_j,x_t\rangle<1-\delta.
\]
The action
     $u_j$
obviously belongs to the cap \(C_j\), and hence, remains feasible if the adversary does not impose the \(j\)\textsuperscript{th} cut $H_j$.  Moreover, $f_t(u_j)=-1$. Therefore, for every round in phase $j,$ we have 
\[
\begin{aligned}
        f_t(x_t)-f_t(u_j)
        &=
        -\langle u_j,x_t\rangle+1 > \delta.
\end{aligned}
\]
If the learner avoids choosing any action from \(C_j\) during the entire duration of phase $j$, the adversary could keep the action 
\(u_j\) feasible up to round $T$ and reveal zero losses and zero constraints after the end of phase $j$.  In this valid problem instance, we now choose \(u_j\) to be a feasible comparator and compute the regret of the algorithm against this action.

Since each loss is $1$-Lipschitz on a set of diameter \(2\), each of the previous \(P_j\) rounds can contribute a regret of at least $-2$.  Thus the regret against the action
\(u_j\) in this instance is at least
\[
        -2P_j+L_j\delta.
\]
By the definition of \(L_j\) given in Eqn.\ \eqref{lj-def}, we have
\[
        L_j\delta
        \ge
        4\bigl(\mathcal R(T)+P_j+1\bigr).
\]
Hence, 
\[
      \Regret(u_j) \geq   -2P_j+L_j\delta
        \ge
        4\mathcal R(T)+2P_j+4
        >
        \mathcal R(T).
\]
This contradicts the regret-budget assumption on \(\mathcal A\).  Therefore the
learner must play an action from the spherical cap \(C_j\) before phase $j$ ends.
\end{proof}
We now continue with the main proof. In view of Claim \ref{claim}, 
let \(\tau_j\) be the first round of phase \(j\) such that $x_{\tau_j}\in C_j$. At this round, after the learner has played \(x_{\tau_j}\), the adversary
reveals the affine constraint function
\[
        g_{\tau_j}(x)
        :=
        \langle u_j,x\rangle-\beta.
\]
By definition, the feasible region for this constraint, defined as $g_{\tau_j}(x) \leq 0,$ is
exactly the half-space \(H_j\) given by Eqn.\ \eqref{feas-set}.  Since \(x_{\tau_j}\in C_j\), we have
\[
        \langle u_j,x_{\tau_j}\rangle\ge 1-\delta.
\]
Therefore at round $\tau_j,$ the learner incurs a constraint violation of 
\[
\begin{aligned}
        (g_{\tau_j}(x_{\tau_j}))_+
        &=
        \bigl(\langle u_j,x_{\tau_j}\rangle-r\beta\bigr)_+\\
        &\ge
        1-\delta-\beta \equiv \nu
\end{aligned}
\]
Thus phase \(j\) contributes at least \(\nu\) amount of violation to the terminal $\CCV$.

After introducing the cut \(H_j\), all future caps \(C_i\), \(i > j\), remain
feasible by virtue of Lemma~\ref{lem:cone-cap-separation}.  
%Any
%remaining rounds in phase $j$ have identically zero loss and identically zero constraint functions \cmt{need to be careful for the strongly convex case as zero cost functions are not allowed. We can just end phase $j$ though, requiring $P_j$ to be an upper bound to its length.}. 
Repeating this construction for phases \(j=1,\ldots, m\), we obtain
\[
        \CCV_T
        \ge
        m\nu. 
\]
%The theorem states the weaker constant \(\nu G_gD/4\), leaving room for floor
%and large-\(T\) conventions.

It remains only to verify that a total of \(m\) phases fit inside the horizon of length $T$.  
\begin{claim} \label{claim2}
	A horizon of length $T$ contains at least $m$ phases.
\end{claim}

\begin{proof}
Define
\[
        Q_j:=P_j+R(T)+1.
\]
%Since \(r=D/2\),
%\[
%        G_fr\delta=\frac{G_fD\delta}{2}.
%\]
Therefore
\[
\begin{aligned}
        L_j
        &=
        \left\lceil
        \frac{4(\mathcal R(T)+P_j+1)}
        {\delta}
        \right\rceil
        \le
        \frac{4}{\delta}
        \left(
            P_j+ R(T)+1
        \right)+1
        \le
        \left(\frac{4}{\delta}+1\right)Q_j.
\end{aligned}
\]
Hence,
\[
\begin{aligned}
        Q_{j+1}
        =
        P_{j+1}+ R(T)+1
        \leq 
        P_j+L_j+ R(T)+1
        =
        Q_j+L_j
        \le
        \left(\frac{4}{\delta}+2\right)Q_j
        \equiv
        B_\delta Q_j.
\end{aligned}
\]
Thus
\[
        Q_{m+1}
        \le
        B_\delta^m Q_1
        =
        B_\delta^m
        \left(
             R(T)+1
        \right).
\]
By the definition of \(m\), we have 
\[
        B_\delta^m
        \left(
            R(T)+1
        \right)
        \le T.
\]
Therefore
\[
        P_{m+1}\le Q_{m+1}\le T.
\]
Hence, all \(m\) phases fit within the horizon of length $T$.
\end{proof}

It is easy to check that common feasibility holds as the origin satisfies all half-space constraints: $\langle u_j,0\rangle=0\le \beta.$ This concludes the proof of Theorem \ref{thm:cone-cap-lower-bound}. 
\end{proof}

%\subsection{A spherical-code corollary}

%The preceding theorem becomes especially useful in high dimensions because standard arguments show that exponentially large (in dimension $d$)
%families of near-orthogonal directions exist \cite{vershynin2020high}.
To derive the final $\CCV$ lower bound for the $\COCO$problem, we use a basic fact from high dimensional geometry that says that there exists exponentially many near-orthonormal vectors as stated in the next lemma. The proof is elementary and is included in Appendix \ref{exp-code} for easy reference. 
\begin{lemma}[Nearly-orthonormal vectors in $d$ dimensions\cite{vershynin2020high}]
\label{lem:spherical-code}
For every fixed \(\rho\in(0,1)\), there is a constant \(c_\rho>0\) such that
for every \(d\ge2\), there exist
\[
        M\ge \exp(c_\rho d)
\]
unit vectors \(u_1,\ldots,u_M\in\mathbb S^{d-1}\) satisfying
\[
        |\langle u_i,u_j\rangle|\le\rho,
        \qquad
        i\neq j.
\]
\end{lemma}

\begin{corollary}[High-dimensional cone-cap lower bound]
\label{cor:high-dimensional-cone-cap-lower-bound}
Fix \(0\le \rho, \delta \le 1\) such that
\[
        \rho+\sqrt{2\delta}<1-\delta.
\]
There are constants \(c,c'>0\), depending only on \(\rho,\delta\), such that
\[
        V_{\mathcal P_{\rm cap}}(\mathcal R,T)
        \ge
        c
        \min\left\{
            \exp(c'd),\,
            \left\lfloor
            \log
            \left(
                \frac{T}{\mathcal R(T)/+1}
            \right)
            \right\rfloor_+
        \right\}.
\]
In particular, if
\[
        d\gtrsim \log\log T,
\]
and the regret budget satisfies
\[
        \mathcal R(T)=\operatorname{poly}(T) \cdot G_fD
\]
with the logarithmic term positive, then the lower bound gives
\[
        V_{\mathcal P_{\rm cap}}(\mathcal R,T)
        =
        \Omega_{\rho,\delta}(G_gD\log T)
\]
up to constants depending on the base of the logarithm and the regret budget.
\end{corollary}


\iffalse
\begin{remark}[Interpretation]
The construction isolates the high-dimensional geometric obstruction.  A cap
\(C_j\) is a small convex cone-like region near the direction \(u_j\).  Because
the directions are almost orthogonal, cutting off one cap by the halfspace
\[
        \langle u_j,x\rangle\le r(\rho+\sqrt{2\delta})
\]
does not affect any other cap.  Losses force the learner toward the current cap;
the constraint then removes it.  Thus each phase contributes a constant amount
of violation, and the number of phases is controlled by the number of
well-separated directions and by the regret-budget forcing time.
\end{remark}
\fi

